Fast Jacobian-Vector Product for Deep Networks

Jacobian-vector products (JVPs) form the backbone of many recent developments in Deep Networks (DNs), with applications including faster constrained optimization, regularization with generalization guarantees, and adversarial example sensitivity assessments. Unfortunately, JVPs are computationally expensive for real world DN architectures and require the use of automatic differentiation to avoid manually adapting the JVP program when changing the DN architecture. We propose a novel method to quickly compute JVPs for any DN that employ Continuous Piecewise Affine (e.g., leaky-ReLU, max-pooling, maxout, etc.) nonlinearities. We show that our technique is on average $2\times$ faster than the fastest alternative over $13$ DN architectures and across various hardware. In addition, our solution does not require automatic differentiation and is thus easy to deploy in software, requiring only the modification of a few lines of codes that do not depend on the DN architecture.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/0-intro.tex <==
\section{Introduction}




==> sections/1-related_work.tex <==
\section{Related Works}


{\bf Max-Affine Spline Deep Networks.}~
Denote the input-output DN mapping as $f:\mathcal{X}\mapsto \mathcal{Y}$ with $\mathcal{X}$ the DN input space $\mathbb{R}^D$ and $\mathcal{Y}$  the prediction space such as $\mathbb{R}$ for univariate regression. 
Collect the parameters of each DN layer in $\mathcal{W}_{\ell}$, which in general corresponds to $\mathbb{R}^{D_{\ell}\times D_{\ell-1}}$.

Some key architectures that we focus on in this paper are given below.
While we define the various layers using the convolution operator $\bC_{\ell}$, the fully connected operator $\bW_{\ell}$ can also be used.
{\em ConvNet} layers \cite{lecun1995convolutional} consist of a convolution operator with parameters $\bC_{\ell}, b_{\ell}$ followed by an activation nonlinearity $\sigma$.
A key result for this paper is as follows. Define a {\em Max-Affine Spline Operator} (MASO) as
\begin{align}
f^{\ell}(\bz) = \max_{r=1,\dots,R}\left(\bW^{\ell}_r \bz+\bb^{\ell}_r\right),\label{eq:explicit_layer}
\end{align}
with the maximum taken coordinate-wise. 


The key result of interest is that any DN layer $f^{\ell}$ constructed from any number of affine transformation and a final (single) continuous piecewise linear operator can be written as a MASO.\cite{reportRB,balestriero2018spline}.
For illustration, layers with 
(leaky) ReLU or absolute value 
activation functions, we have $R=2$ and $D^{\ell}$ a diagonal matrix with entries ${\eta, 1}$.
For leaky-ReLU with leakiness $\eta>0$, ReLU with $\eta=0$, and absolute value with $\eta=-1$.



{\bf Deep Network Partition.} Whenever a DN can be expressed as a MASO, it becomes a continous piecewise affine mapping \cite{unser2018representer} with an inherent input space partition and per region affine mappings. 
By the form of (\ref{eq:explicit_layer}) it is clear that there exists an underlying layer input space partition based on the realization of the maximum operator.


\begin{defn}
\label{def:partition}
A collection  $\Omega=\{\omega_1,\dots,\omega_R\}$ of subsets of a space $\mathcal{X}$ is called a 
\emph{partition} if the $R$ subsets  $\omega_r$ (called \emph{regions}) have disjoint interiors and their union makes up the entire
space $\mathcal{X}$.
%$\cup_{r=1}^R \omega_r=\mathcal{X}$ 
\end{defn}


It is possible to express this partition as a power diagram (a generalization of Voronoi diagrams) subdivision with convex (polytopal) regions \cite{balestriero2019geometry}. This partition $\Omega$ of the the DN input space is composed of  non-empty and non-intersecting regions $\omega$ that collectively represent the entire DN input space leading to the following DN input-output form
\begin{align}
    f(\bx)=\sum_{\omega \in \Omega}(A_{\omega}\bx+\bb_{\omega})\Indic_{\bx \in \omega}
\end{align}
where the above parameters denote the $\omega$-associated affine parameters. The crucial result being that the internal weights of the DNs are paired with the DN partition $\Omega$. As pruning impacts those weights directly, this will offer us in the next section a novel way to study pruning into DNs.




\textbf{Network Pruning.} Pruning is a widely used DNNs compression technique for reducing activated neurons \citep{liu2018rethinking,lecun1990optimal}. The common pruning schemes adopt a three-step routine of 1) training a large and dense model, 2) pruning it, and 3) then retraining the pruned model to restore performance, and these three steps can be iterated to get a highly-sparse network \citep{han2015deep}. Within this routine, different pruning methods vary primarily in their choices of pruning criteria, granularity, and scheduling \citep{liu2018rethinking,blalock2020state}. 
\citep{frankle2019lottery} first hypothesises there exist small sub-networks, called winning tickets, can restore the comparable test accuracies of dense networks.
\citep{you2020drawing} finds that critical sub-networks (connectivity) can be identified in the early training stage of dense networks, called early-bird (EB) tickets, and further propose a more efficient pruning scheme.
However, the network pruning literature lacks of a theoretical analysis regarding the early critical patterns of sub-networks, which is a direct motivation for us to leverage the spline theory \citep{balestriero2018spline} for representing pruning and analyzing from the decision boundary perspective.


FYI: The pruning criteria includes the way your mentioned before, one can prune unnecessary neurons according to the weight magnitudes or other hand-crafted criteria. The pruning granularity can be roughly divided into two categories: structured and unstructured, the unstructured methods consider all neurons equally and prune them accordingly, while structured ways prune parameters in group, e.g., filter-wise, channel-wise pruning.


% different pruning ways
\textbf{Pruning Goal.} 
Taking as input the dense networks parameterized with specific parameters $f(x; W)$, network pruning methods apply binary masks $m \in \{0, 1\}$ (can be learnable) to the weight parameters to achieve sparsification. The produced sparse networks $f(x, m \odot W)$ are supposed to be fully expressive and can achieve comparable or even better accuracies as compared to their dense counterparts when trained in isolation.

\textbf{SOTA Practice.}
The pruning schemes adopt a three-step routine of 1) training a large and dense model, 2) pruning it, and 3) then retraining the pruned model to restore performance, and these three steps can be iterated to get a highly-sparse network \citep{han2015deep, frankle2019lottery}.

\textbf{Unstructured Pruning.} One major branch of network pruning methods is the unstructured weight pruning, it prunes unimportant connections according to the weight magnitudes. The common practice is to collect weights globally or in a layer-wise manner and then sort them in a descending order for pruning a proportion of small-magnitude weights.
Such pruning methods are usually conducted after fully training the dense network, and can also be iterated several times to find a highly sparse network \citep{han2015deep, frankle2019lottery}.
Iterative pruning during training process is also discussed in \citep{evci2019rigging}.
However, one significant drawback of unstructured weight pruning methods is that the resulting sparse weight matrices require dedicated hardware co-design to speedup, otherwise they cannot show any benefit in terms of the efficiency metrics.

\textbf{Structured Pruning.} 
In contrast, structured pruning methods prune a group of weights, leading to the direct dimensional reductions in weight matrices.
For example, node pruning in fully-connected layer can be viewed as one kind of structured pruning methods, since it prunes all the weights related to that particular node simultaneously.
The case can also generalized to convolutional layers.
\citep{he2018soft} proposes to prune and recover filters during training process;
\citep{chin2020legr} prunes the bottom-ranked filters by learning a global ranking of all filters.
\citep{liu2017learning} imposes a $l$-1 penalty term to learn the ``importance score'' of each channel and prune unimportant channels directly.
Although the different pruning granularities have been discussed, the SOTA methods are still hard to determined due to a lack of standardized benchmarks and metrics \citep{blalock2020state}.

Regardless of pruning methods, the trade-offs between efficiency (how many parameters are left or how many computational costs are needed) and accuracy are generally exist.

==> sections/2-methods.tex <==
\section{Winning Tickets and Deep Networks Initialization}


We propose in this section a simple example illustrating the concept of winning tickets and its link with the difficulty of optimizing a non overparametrized MASO DN.


\begin{figure}[t]
    \centering
    \begin{minipage}{0.035\linewidth}
    \rotatebox{90}{test accuracy}
    \end{minipage}
    \begin{minipage}{0.5\linewidth}
    \centering
    mixture of $40$ Gaussian
    \includegraphics[width=\linewidth]{figures/over.pdf}\\
    number of initial clusters
    \end{minipage}
    \begin{minipage}{0.4\linewidth}
    \caption{The number of final cluster is always the same and is exactly the number of Gaussians.}
    \label{fig:kmean}
    \end{minipage}
\end{figure}


\subsection{The Initialization Dilemma}

Let consider the simple unidimensional sawtooth like function given in Fig.~\ref{fig:sawtooth} with $P$ peaks. We now demonstrate that in the special case of a single hidden layer with ReLU activation you must have at least $2P$ units, one weight configuration being $[\bW_{1}]_{1,k}= 1, [\bb_{1}]_k=-k$ with $k=1,\dots,D_1$ and $[\bW_2]_{1,1}=1,[\bW_2]_{1,k}(-2)^{(k-1)\%2}, k=2,\dots,D_1$.
Now, at initialization, if the DN has only $2P$ units, it is very unlikely that the initialization will allow training to converge to the correct DN as some of the splines will be poorly initialized possibly concentrating multiple ones on a single peak. In the presence of a gradient based optimization, a poor local minima can not be escaped (this can be seen easily as the gradient will be $0$ for all weights).
However, with a very wide DN thus involving overparametrization, the larger number of random weight initialization will allow for a higher chance of starting with a well positioned spline from this convergence to the true function will be achieved. This convergence will involve (at least) the splines that were initialized at the correct positions, those are the ones corresponding to the winning ticket DN.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/over_width.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}



\begin{remark}
Winning tickets are the result of employing overly parametrized DNs compared to the task at hand.
\end{remark}

\begin{remark}
Overly parametrized DNs are needed as current optimization techniques can not escape poor local minima, and smart DN initialization (near good local minima) is not known.
\end{remark}

We further support the above point in the following section where we demonstrate how the absence of good initialization coupled with non optimal optimization problem impacts performances unless overparametrization is used, in which cased winning tickets naturally emerge.

\subsection{Winning Tickets in other ML algorithms} 

this initialization issue being countered by overparametrization is not unique to DNs. In fact we propose here a simple illustration with the K-means algorithms in which we propose to initialize with much more centroids than needed, then during learning the closest centroids are gradually pruned such that the final K-means all have the same number of centroids which is the true number of gaussians. We demonstrate that in the context of random initialization, this technique guarantees to always have a K-means that converges to the true centroids. We depict this result in Fig.~\ref{fig:kmean}.

As a result, we see that in the current regime of DN architecture and optimization, we need to overparametrize to allow some of the components to be initialized correctly, from which we can prune the other ones keeping only the winning ticket DN.

\subsection{How to better initialize}


We saw in the previous section that the concept of winning tickets emerges from the need to overparametrize which is needed to reach good performances. We also saw that this concept is not unique to DNs. However, many other ML algorithms do not need to overparametrize due to the implementation of more complex initialization techniques such as kmeans++ for kmeans, kmeans for GMM and so on. We now demonstrate if such smart initialization can occur in current DNs.


TODO: study layer wise training, pretraining

conclusion: it is hard to do clever initialization in complicated DN, much simpler to overparametrize and prune. We thus study the impact of pruning into the DN geometry in the next section


\section{Pruning Impact on the Deep Network Partition}


\begin{figure}[t]
    \centering
    \begin{minipage}{0.035\linewidth}
    \rotatebox{90}{weight pruning \hspace{1cm} node pruning}
    \end{minipage}
    \begin{minipage}{0.945\linewidth}
    \includegraphics[width=\linewidth]{figures/2d_case.pdf}
    \includegraphics[width=\linewidth]{figures/2d_case_other.pdf}
    \end{minipage}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}


